Rotation Initialization and Stepwise Refinement for Universal LiDAR Calibration

Autonomous systems often employ multiple LiDARs to leverage the integrated advantages, enhancing perception and robustness. The most critical prerequisite under this setting is the estimating the extrinsic between each LiDAR, i.e., calibration. Despite the exciting progress in multi-LiDAR calibration efforts, a universal, sensor-agnostic calibration method remains elusive. According to the coarse-to-fine framework, we first design a spherical descriptor TERRA for 3-DoF rotation initialization with no prior knowledge. To further optimize, we present JEEP for the joint estimation of extrinsic and pose, integrating geometric and motion information to overcome factors affecting the point cloud registration. Finally, the LiDAR poses optimized by the hierarchical optimization module are input to time synchronization module to produce the ultimate calibration results, including the time offset. To verify the effectiveness, we conduct extensive experiments on eight datasets, where 16 diverse types of LiDARs in total and dozens of calibration tasks are tested. In the challenging tasks, the calibration errors can still be controlled within 5cm and 1{\deg} with a high success rate.

==> chapters/a6.registration_ds.tex <==
\section{Calibration with Data Sequences}
\label{sec:reg_datasequences}
As previously mentioned in Sec.~\ref{sec:formulation}, we model the calibration problem as a point cloud registration problem. There are various methods for performing point cloud registration. However, in this paper, we do not enhance specific registration algorithms; instead, we investigate what data, when fed into the registration algorithms, yields the best outcomes.\xnote{Why choose ICP? Why tell the baseline method? If we use it to build our method, perhaps we need not emphasize it. If we compare with it, we can address it in the experiments.}\dnote{I have revised the phrasing and moved the words on ICP to Sec.~\ref{sec:exp}.}

% By reversing the roles of the source and target in the registration process, we can obtain several different registration methods.

% In this section, we will analyze each possible registration method step by step, pointing out the measurement error or system error that each method may contain. Finally, we propose a registration method suitable for the calibration problem that does not involve system errors and can obtain acceptable errors as the sequence grows.
To find a more suitable registration approach for two LiDAR data sequences, i.e., determining which two point clouds are the inputs of registration, we analyze the errors introduced by different inputs in this section. Specifically, the process begins with analyzing two individual frames as inputs, referred to as the scan-to-scan method. Subsequently, the approach of concatenating all data from the sequences to form  maps for registration, named the map-to-map method, is examined. We also investigate a hybrid strategy, using a map of one LiDAR and an individual frame of the other, which is mentioned in~\cite{mloam}. Finally, incorporating hand-eye calibration, we propose a technique that maintains computational efficiency while minimizing errors, termed \je.

To compare the strengths and weaknesses of different approaches, we adopted the methods from \cite{covariance1, covariance2, covariance3}, classifying potential sources of error in the registration process into five categories: wrong convergence, wrong initialization, sensor noise and bias, under-constrained situations, and intrinsic randomness of ICP. However, in this article, we have made some adjustments. 

In specific, the initialization is uniformly provided by the method introduced in the Sec.~\ref{sec:ri}. Therefore, we don't analyze the errors caused by initialization but only test the outcomes under different initialization errors in the experiment part. Following that, the convergence error and the randomness are inherent characteristics of ICP that cannot be avoided, and thus are not discussed extensively. Moreover, since the goal of this article is to calibrate any two unknown LiDARs, it is difficult to model the noise and bias of the sensors in advance. However, since the input in the subsequent registration process might be processed inputs, such as map-to-map registration mentioned above, we redefine the noise and bias of the sensors in this article, that is, the \textbf{point cloud noise} and \textbf{point cloud bias}. This means that the noise caused by the sensor's noise and bias is defined as the point cloud noise, and the cumulative error introduced by the stitching process is defined as the point cloud bias. Finally, the \textbf{degeneracy} caused by under-constrained situations remains a key observation object. In our experiments, we draw inspiration from the "localizability detection module"~\cite{xicp}, to categorize and statistically analyze the degree of degeneracy, demonstrating the extent to which different methods are affected by this factor. \xnote{This paragraph needs to be reorganized: First, the explanation about the experiment could be removed to the experiment section. Second, perhaps we need a sentence to summarize this paragraph, for example, we first outline some prerequisites. Alternatively, maybe we can move the explanation to the end of this section or scatter it throughout the relevant subsection? Finally, consider the bolded words. Some terms that appear more important in the preceding text remain unbolded, such as \sd, \je, and the method name, scan-to-scan and map-to-map.}

% \subsection{pipeline}
% \label{sec:pipeline}
% As shown in Fig.~\ref{fig:pipeline}, \core is divided into four parts. First, \core supports the calibration task of any two types of depth sensors and takes the data flow of the two sensors as input. Then, the coarse step, i.e., rotation initialization, and the fine step, i.e., joint estimation, form the core function of calibration. 

% In specific, we initialize the rotation part of extrinsic parameters through two steps. Similar to CROON~\cite{CROON}, We noticed that the data from the depth sensor usually contains a large number of points on the ground in autonomous driving scenarios, and the initial value of $roll$ and $pitch$ can be obtained easily by utilizing this feature. Next, we borrow the idea of the state-of-the-art method of place recognition, Scan Context~\cite{scancontext}, to initialize $yaw$. The rotation initialization will be detailed in Sec.~\ref{sec:ri}. 

% To refine the calibration result, the two frames of point clouds with initial rotation values are optimized by the joint estimation of the motion of sensors and the extrinsic parameters, which will be deduced and analyzed in Sec.~\ref{sec:je}.

% Finally, the precise $\mathbf{C}$ is output, with a by-product, i.e., the more accurate motion estimation
% $\mathbf{T}^*_a$.

% \subsection{Rotation Initialization}

% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width = \linewidth]{fig/planealign.pdf}
% 	\caption{The calibration result in simulated environment. 
% 	}
% 	%Examples of \metric and \core.}
% 	\label{fig:planealign}
% \end{figure}

% Having a good initial value is important for solving non-convex optimization problems. Similarly, a good initial guess can make the registration problem in the calibration converge quickly. The most traditional method usually needs to manually specify the initial value, which requires people to have sufficient sensitivity to the three-dimensional coordinates. In the past few years, motion-based initialization methods have dominated. But these methods usually requires constructing an accurate pose estimation algorithm for each sensor, and needs the experimental platform to have  sufficient motion, which provides enough constraints. In this paper, we borrow the algorithm of place recognition and use it in registration initialization.

% It is worth noting that in the calibration problem, the translation between sensors is usually not very large, for the reason that the sensors are all equipped in the same experimental platform. On the other hand, the orientation angle of sensors are often quite different in order to allow the FOV of the sensors to cover the entire space. 
% The above facts show that among the extrinsic parameters of 6 DoF, the translation part already has a good initial value, while the rotation part does not. 
% In this paper, we focus on the initialization of the rotation simplify the initialization problem of 6 DoF to 3 DoF.

% Additionally, we split the rotation estimation task into two sub-problems, which greatly reduces the search space of the initial values and speeds up the initialization. First, we estimate the $roll$ and $pitch$, i.e., the rotation around the x-axis and y-axis, and then estimating $yaw$ for rotation around the z-axis. 

% \subsubsection{Roll and Pitch}
% \subsubsection{Yaw}

\begin{figure}[t]
	\centering
	\subfigure[Scan to scan] {\includegraphics[width = 0.45\linewidth]{fig/refine1.pdf}\label{fig:ref1}}
	\subfigure[Map to map] {\includegraphics[width = 0.45\linewidth]{fig/refine2.pdf}\label{fig:ref2}}
	\subfigure[Scan to map] {\includegraphics[width = 0.45\linewidth]{fig/refine1.pdf}\label{fig:ref3}}
	\subfigure[Registration and Hand-Eye] {\includegraphics[width = 0.45\linewidth]{fig/refine1.pdf}\label{fig:ref4}}
	\caption{Comparison of different refinement methods. 
	}
	%Examples of \metric and \core.}
	\label{fig:je}
\end{figure}



\subsection{Calibration by Scan-to-Scan Registration}
Through scan-to-scan registration~\cite{CROON}, we form the most direct calibration method\xnote{What is direct? Simple? What does indirect look like? }. Each calibration takes the scan from two LiDARs at the same time as input, and outputs the transformation between them, as follows:
\begin{equation}
\mathbf{C}^* = \mathop{\arg\min}_\mathbf{T} \ \ \|d(^t\mathcal{S}_a, \mathbf{T}(^t \mathcal{S}_b))\|^2.\\
\end{equation}
This approach attempts to calculate the relationship between one frame and another without being influenced by other factors, meaning its point cloud bias is relatively small. However, every advantage has its disadvantage; since only a single frame of data provides constraints, the impact of noise and degeneracy becomes significant.
% \begin{itemize}
%     \item Sparsity of the Laser Point Clouds: LiDAR sensors differ in their resolution and scanning mechanisms, leading to variances in point cloud density. Sparse point clouds have fewer points for establishing correspondences, increasing the likelihood of inaccurate registrations. This sparsity becomes even more problematic in environments where significant portions contain few features, making it difficult to find reliable matching points.
%     \item Diversity of the Environments and Degraded Scenes: Environmental diversity introduces variability in the features and structures captured by LiDAR scans. In highly dynamic or cluttered environments, identifying consistent, stable features for registration can be challenging. Furthermore, degraded scenes, such as those with low visibility, occlusions, or absence of distinctive landmarks, can severely limit the registration accuracy. The presence of dynamic objects can also introduce non-static elements into the scans, compounding the complexity of finding a correct alignment.
% \end{itemize}


\subsection{Calibration by Map-to-Map Registration}
To overcome the limitations of the above method, we attempt to register and align  frames in the data sequence from a single LiDAR for the purpose of constructing a map for each LiDAR, that is,
\begin{equation}
^t\mathcal{M}_a = \bigcup_{i \in [0, t]}~^i\mathbf{P}_a ( ^i\mathcal{S}_a), ~
^t\mathcal{M}_b = \bigcup_{i \in [0, t]}~^i\mathbf{P}_b ( ^i\mathcal{S}_b).
\end{equation}

Since the maps use the coordinate system of the first frame of the LiDAR, calculating the pose between the two maps allows for the acquisition of the extrinsic parameters between the two LiDARs~\cite{small_fov}:
\begin{equation}
\label{eq:map_calib}
\mathbf{C}^* = \mathop{\arg\min}_\mathbf{T} \ \ \|d(^t\mathcal{M}_a, \mathbf{T}(^t \mathcal{M}_b))\|^2.\\    
\end{equation}
In this case, due to the increase in points for registration, the issue of scene degradation can be mitigated in non-extreme cases. However, the pose error of each LiDAR accumulates over time, leading to the map distortion, i.e., the point cloud bias. To specifically analyze how this cumulative error affects the solution of Eq.~\ref{eq:map_calib}, we split the poses $^i\mathbf{P}_a$ and $^i\mathbf{P}_b$ into two parts, i.e., the ground truth transformation and the noise, denoted as  $^i\mathbf{P}_a, ^i\mathbf{P}_b$ and $^i\mathbf{P}_a^{'}, ^i\mathbf{P}_b^{'}$. According to Eq.~\ref{eq:hand_eye_eq}, $^i\mathbf{P}_a$ and $^i\mathbf{P}_b$  satisfy the following equation:
\begin{equation}
\label{eq:replace}    
^i\mathbf{P}_b = \mathbf{C}^{-1}\cdot ~^i\mathbf{P}_a \cdot \mathbf{C}.
\end{equation}
Due to the complexity of directly analyzing the errors in aligning two maps, we take the t-th frame as an example, representing the potential maximum error, as errors accumulate over time.
The Eq.~\ref{eq:map_calib} can be rewritten as\dnote{The derivation is not very rigorous.}:
\begin{equation}
\label{eq:map_cali_re}
\mathbf{C}^* = \mathop{\arg\min}_\mathbf{T} \ \ \|
d(( ^t\mathbf{P}_a^{'} \cdot ^t\mathbf{P}_a)( ^t\mathcal{S}_a), 
(\mathbf{T}\cdot ^t\mathbf{P}_b^{'} \cdot ^t\mathbf{P}_b ) (^t \mathcal{S}_b))\|^2.
\end{equation}
% \begin{align*}
%     &P_{i}^* = P_{i}^{'}P_{i}\\
%     &P_{i+1}^* = P_{i+1}^{'}P_{i+1}P_{i}^*\\
%     &^i\mathbf{P}_a = ^0_i\mathbf{T}_a = ^0_1\mathbf{T}_a \cdot ^1_2\mathbf{T}_a \dots  ^{i-1}_i\mathbf{T}_a.\\
%     &^i\mathbf{P}_a^* = ^0_i\mathbf{T}_a = ^0_1\mathbf{T}_a^{'}~^0_1\mathbf{T}_a \cdot ^1_2\mathbf{T}_a{'}~^1_2\mathbf{T}_a \dots  ^{i-1}_i\mathbf{T}_a^{'}~^{i-1}_i\mathbf{T}_a = ^iP_a^{'}^iP_a.\\
%     &^{i+1}\mathbf{P}_a^* = ^0_i\mathbf{T}_a = ^0_1\mathbf{T}_a^{'}~^0_1\mathbf{T}_a \cdot ^1_2\mathbf{T}_a{'}~^1_2\mathbf{T}_a \dots  ^{i-1}_i\mathbf{T}_a^{'}~^{i-1}_i\mathbf{T}_a\cdot^{i}_{i+1}\mathbf{T}_a^{'}~^{i}_{i+1}\mathbf{T}_a.\\
% \end{align*}
Bring Eq.~\ref{eq:replace} into Eq.~\ref{eq:map_cali_re}, the optimal solution of the calibration result is:
\begin{equation}
\label{eq:map_wrong}    
\mathbf{C}^* = ^i\mathbf{P}_a^{'} \cdot \mathbf{C} \cdot ^i\mathbf{P}_b^{'-1}.
\end{equation}
As can be seen from the above equation, the extrinsic parameter $\mathbf{C}^*$ obtained by solving Eq.~\ref{eq:map_calib} will increasingly deviate from the true value $\mathbf{C}$ as the cumulative error in pose accumulates.


\subsection{Calibration by Scan-to-Map Registration}
Due to the drawbacks of the two methods mentioned above, some multi-LiDAR calibration method~\cite{mloam, lidar_link} has adopted a balanced approach, namely scan-to-map registration. Similar to Eq.~\ref{eq:map_calib}, we define this method as
\begin{equation}
\label{eq:scan_map_calib}
\mathbf{C}^* = \mathop{\arg\min}_\mathbf{T} \ \ \|d(^t\mathcal{M}_a, \mathbf{T}(^0 \mathcal{S}_b))\|^2.\\    
\end{equation}
Following the analysis of the previous step, we can conclude that the optimal solution for the calibration result is
\begin{equation}
\label{eq:scan_map_wrong}    
\mathbf{C}^* = ^i\mathbf{P}_a^{'} \cdot \mathbf{C},
\end{equation}
whose error is smaller than that of the map-to-map method, but is still affected by the cumulative pose error of LiDAR a.
\subsection{Calibration by Registration and Hand-Eye}
\label{sec:je}
To integrate the advantages of both the scan-to-scan and map-to-map methods while mitigating their drawbacks, we consider incorporating hand-eye calibration constraints. This approach aims to minimize the impact of cumulative pose errors on the calibration results. Specifically, our method is divided into two phases: pose estimation phase and calibration phase. During the pose estimation phase, we utilize the principles of hand-eye calibration, combining the extrinsic parameters and the motion of LiDAR a to derive the motion of LiDAR b. This means that the problem of pose estimation is as follows:
\begin{equation}
\begin{aligned}
\label{eq:je_odom}
   ^i\mathbf{P}^*_a = \mathop{\arg\min}_\mathbf{T} (\ \ &\|d(^t\mathcal{M}_a, \mathbf{T}(^t \mathcal{S}_a))\|^2 + \\
   &\|d(^t\mathcal{M}_b, (\mathbf{C}^{*-1} \cdot \mathbf{T} \cdot \mathbf{C}^*)(^t \mathcal{S}_b))\|^2), \\
\end{aligned}
\end{equation}
where the pose of LiDAR b is replaced by $\mathbf{C}^{*-1} \cdot \mathbf{^i\mathbf{P}^*_a} \cdot \mathbf{C}^*$ and the $\mathbf{C}^{*}$ is either the initial value or the result that is continuously updated during iterations.
In the calibration phase, we continue to use the objective function outlined in Eq.~\ref{eq:map_calib}.

For error analysis, we still divide the solved variables into two parts: the error and the true value, namely 
\begin{equation}
\label{eq:pa}
^i\mathbf{P}^*_a = ^i\mathbf{P}_a^{'} \cdot ^i\mathbf{P}_a; ~~\mathbf{C}^* = \mathbf{C}^{'} \cdot \mathbf{C}.
\end{equation}
Following that, if $^i\mathbf{P}^*_b$ is also expressed as $^i\mathbf{P}_b^{'} \cdot ^i\mathbf{P}_b$, then according to Eq.~\ref{eq:replace}, it can be calculated that
\begin{equation}
\label{eq:error_pb}
^i\mathbf{P}_b^{'} = \mathbf{C}^{-1}\mathbf{C}^{'-1}~^i\mathbf{P}^*_a ~\mathbf{C}^{'}~ ^i\mathbf{P}_a^{-1} \mathbf{C}
\end{equation}
Bring Eq.~\ref{eq:error_pb}  into Eq.~\ref{eq:map_wrong}:
\begin{equation}
\label{eq:je_error}    
\mathbf{C}^* = ^i\mathbf{P}_a^{*} \cdot \mathbf{C}^{'-1} \cdot ^i\mathbf{P}_a^{*-1} \cdot \mathbf{C}^{'} \cdot \mathbf{C}
\end{equation}
By combining the latter halves of Eq.~\ref{eq:pa} and Eq.~\ref{eq:je_error}, we can obtain
\begin{equation}  
^i\mathbf{P}_a^{*} \cdot \mathbf{C}^{'-1} \cdot ^i\mathbf{P}_a^{*-1} = \mathbf{I}
\end{equation}
which holds true if and only if $\mathbf{C}^{'}$ is an identity matrix. In other words, the $\mathbf{C}^*$ obtained in this manner is unaffected by the error pose estimation. It's important to note that the $\mathbf{C}^*$ calculated by this method may not always match the actual extrinsic parameters. This only demonstrates that we have eliminated the influence of point cloud bias among the factors affecting registration. Due to the inherent characteristics of ICP, scene degeneracy, and point cloud noise, errors still exist. However, these errors tend to decrease with the accumulation of multiple frames, as we have demonstrated in our experiments.

% \begin{align*}
%     1.^i\mathbf{P}_b &= \mathbf{C}^{-1}\cdot ~^i\mathbf{P}_a \cdot \mathbf{C}\\
%     2.^i\mathbf{P}^*_b &= ^i\mathbf{P}_b^{'} \cdot ^i\mathbf{P}_b \\
%     3.&= \mathbf{C}^{*-1} \cdot ^i\mathbf{P}_a^* \cdot \mathbf{C}^*\\
%     4.^i\mathbf{P}_b^{'} \mathbf{C}^{-1}\cdot ~^i\mathbf{P}_a \cdot \mathbf{C}&= \mathbf{C}^{*-1} \cdot ^i\mathbf{P}_a^{'} \cdot ^i\mathbf{P}_a  \cdot \mathbf{C}^{'} \cdot \mathbf{C}\\
%     5.^i\mathbf{P}_b^{'} &= \mathbf{C}^{*-1} \cdot ^i\mathbf{P}_a^{'} \cdot ^i\mathbf{P}_a  \cdot \mathbf{C}^{'} \cdot ^i\mathbf{P}_a^{-1} \cdot \mathbf{C}\\
%     6.^i\mathbf{P}^*_b &= ^i\mathbf{P}_b^{'} \cdot ^i\mathbf{P}_b\\
%     7.\mathbf{C}^* &= \mathbf{C}^{'} \cdot \mathbf{C}\\
%     &= ^i\mathbf{P}_a^{'} \cdot \mathbf{C} \cdot ^i\mathbf{P}_b^{'-1} \\
%     8.  \mathbf{C}^{'} \cdot \mathbf{C} ^i\mathbf{P}_b^' &= ^i\mathbf{P}_a^{'} \cdot \mathbf{C}\\
%     9. ^i\mathbf{P}_a^{'} \cdot ^i\mathbf{P}_a  \cdot \mathbf{C}^{'} \cdot ^i\mathbf{P}_a^{-1} \cdot \mathbf{C} &= ^i\mathbf{P}_a^{'} \cdot \mathbf{C}\\
%     10. ^i\mathbf{P}_a^{'} \cdot ^i\mathbf{P}_a  \cdot \mathbf{C}^{'}&= ^i\mathbf{P}_a^{'} \cdot ^i\mathbf{P}_a
% \end{align*}



% \begin{align*}
%     P_1^{c_1} &= P_2^{c_1} \\
%     C^{-1}\Delta C CP &= T^{-1} C^{-1}\Delta C CTP\\
%     C^{-1}\Delta C C &= T^{-1} C^{-1}\Delta C CT\\
%     CTC^{-1}\Delta C&= \Delta C CTC^{-1}\\
%     CTC^{-1}\Delta CC&= \Delta C CT
% \end{align*}



% The second part is:
% \begin{equation}
% \begin{aligned}
%     \mathbf{J}_p = \frac{\partial\, \mathbf{C}^{-1}\mathbf{T}\mathbf{C}p}{\partial \delta \xi} &= \lim_{\delta \xi \rightarrow 0}\frac{\mathbf{C}^{-1}exp(\delta \xi)\mathbf{T}\mathbf{C}\mathbf{p} - \mathbf{C}^{-1}\mathbf{T}\mathbf{C}\mathbf{p}}{\delta \xi}\\
%     &=\mathbf{R}^{\mathbf{C}^{-1}}_{3\times3}\begin{bmatrix} \mathbf{I}_{3\times3}  & -[\mathbf{R}^\mathbf{T}\mathbf{R}^\mathbf{C}  \mathbf{p} + \mathbf{R}^\mathbf{T} \mathbf{t}^\mathbf{C} + \mathbf{t}^\mathbf{T}]_\times \\ \mathbf{0}_{1\times3} & \mathbf{0}_{1\times3} \end{bmatrix}
% \end{aligned}
% \end{equation}

==> chapters/a7.hierarchical_op.tex <==
\section{Hierarchical Optimization}
\label{sec:ho}
\begin{figure*}[t]
	\centering
	\includegraphics[width = \linewidth]{fig/hba.png}
	\caption{place holder}
	\label{fig:hba}
\end{figure*}

In this section, we first aim to minimize the cumulative error introduced in the previous session\xnote{in Section XXX}by employing a hierarchical optimization backend. Subsequently, after acquiring the more accurate poses for each frame from every LiDAR, a time synchronization method is devised to calculate the time offset when capturing data from different LiDARs, with the expectation of providing more useful information for subsequent applications.
\subsection{Pose Refinement by Hierarchical Optimization}
In the field of SLAM, a common method used for backend optimization involves using factor graphs to optimize all variables together, achieving global consistency. However, this approach typically optimizes only at the level of poses, overlooking the constraints introduced by the point cloud itself. Inspired by HBA~\cite{hba}, we employ a similar hierarchical optimization here to achieve more accurate poses for each data frame. 

Specifically, during the first layer of optimization, radar frames captured within a specified window size form a local submap with poses generated during the registration process. The relative poses among the frames within this submap are considered reliable, and the submap's pose is represented by the pose of the first frame, while the poses of the remaining frames are not optimized within the factor graph.\xnote{We do not use the factor graph optimization method, but mention it here. So, we may need to describe the relationship between the method of factor graph optimization and hierarchical optimization at the beginning.} In the second and above layers of optimization, a similar process is conducted. The difference is that the relative poses between each submap are further optimized by the scan-scan registration algorithm. Finally, the relative poses between adjacent submaps are incorporated as factors, used to construct a factor graph, which is then optimized further by GTSAM~\cite{gtsam}. The structure of HBA is illustrated in Fig.~\ref{fig:hba}.

The biggest issue with using hierarchical optimization is its significant memory usage, for the reason that each layer replicates the data. Despite the appropriate downsampling, memory consumption will quickly increase as the number of LiDAR frames increases.\xnote{Do we need to use data to illustrate it?} To alleviate the storage load\xnote{I think storage is different from memory. Do not confuse them}, a filtering strategy, i.e., PFilter, has been adopted from our previous work~\cite{duan2022pfilter}.\xnote{Can we say this is our previous work? Do we need to state it in a third-person perspective?} The core idea of PFilter is evaluating whether a point is persistent or transient by observing its distribution across consecutive frames, extracting a point cloud subset that is more efficient for registration, thereby reducing memory usage, accelerating and enhancing precision. PFilter is executed at each layer of registration, reducing the memory consumption of each layer. \xnote{Do we have experiments about it?}

In addition, since the registration process within each submap is independent, it is suitable to use parallel computing to accelerate the process. To achieve that, we maintain a thread pool and a task queue. When each submap needs to be stitched, the task is added to the task queue and the idle thread will retrieve tasks from the task queue. \xnote{Why should we do it? Not because it's suitable, but because we need it.}
\subsection{Time Synchronization}
\begin{figure}[t]
	\centering
	\includegraphics[width = \linewidth]{fig/timesyn.pdf}
	\caption{todo}
	\label{fig:time_syn}
\end{figure}

After \je and \ho, each LiDAR frame's pose is as accurate as possible. However, as illustrated in Fig.~\ref{fig:time_syn}, in the absence of time synchronization for the LiDAR pairs, the pose between two aligned frames from two LiDARs, denoted as $^i \textbf{C}^r= ^i \textbf{P}_a^{-1}~^i\textbf{P}_b$ here, is not the actual extrinsic parameters, denoted as $^i \textbf{C}^*$ here, between the LiDARs.\xnote{Not the actual extrinsic parameters, what is the result? What happened?} Therefore, we propose a method for time calibration to estimate the temporal offset between different LiDARs.

It's worth noting that we assume a consistent frame rate for the LiDAR, meaning the time offset is a constant value. Moreover, between adjacent frames from the same LiDAR, the motion status remains consistent, allowing us to obtain the position at any given moment through interpolation. \xnote{We have a paragraph at the beginning of Sec.\ref{sec:reg_datasequences} to say some assumptions. Do we need to merge this paragraph with it? }

More specifically, we hypothesize the time offset between two LiDARs as $\delta t$ and the interval of LiDAR capturing data as $t_f$. The ratio between $\delta t$ and $t_f$ is denoted as $\alpha=\frac{\delta t}{t_f}$. The pose bias caused by the time offset is denoted as 
\begin{equation}
    ^i \textbf{T}_b^\delta=\alpha~^{i-1} \textbf{P}_{b}^{-1}~ ^i \textbf{P}_b,\\
\end{equation}
where $\alpha$ means interpolating the pose. 
The translation part is linear interpolation under constant velocity assumption, while the rotation part is spherical linear interpolation (Slerp)~\cite{dam1998quaternions}. 
Following that, the triangular relationship in the Fig.~\ref{fig:time_syn} can be expressed as:
\begin{equation}
  ^i \textbf{C}^*~ ^i \textbf{T}_b^\delta = ^i \textbf{C}^r
  \label{eq:relationship}
\end{equation}
Substituting $^i \textbf{T}_b^\delta$ and $\textbf{C}^r_i$ into Eq.~\ref{eq:relationship}, we get
\begin{equation}
    ^i \textbf{C}^* = ^i \textbf{P}_a^{-1}~^i\textbf{P}_b (\alpha~^{i-1} \textbf{P}_{b}^{-1}~ ^i \textbf{P}_b)^{-1}.
\end{equation}

To find the optimal extrinsic parameters $\textbf{C}^*$ and time-offset ratio $\alpha$, we model the search process as a problem of minimizing the variance of $^i \textbf{C}^*$, i.e.,


\begin{align}
    \alpha ^* & = \mathop{\arg\min}_\alpha Var(\mathbb{C}^*|\alpha), \label{eq:var}\\
    \textbf{C} ^* & = Mean( \mathbb{C}^*|\alpha ^*) \label{eq:mean}
\end{align}
where $\mathbb{C}^* = \{^1 \textbf{C}^*, ^2 \textbf{C}^*, \cdots, ^i \textbf{C}^*\}$, and the $\textbf{C}^*$ is the final output of the whole algorithm. \xnote{It seems that we haven't utilized \core to describe in the design section.}

==> tables/N_res_time.tex <==
\begin{table}[t]
\caption{The relationship between the number of points $N$, resolution, and the time required for one rotation\dnote{move to exp}}
\label{table:N_res_time}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\begin{tabular}{|c|>{\centering\arraybackslash}p{0.54cm}|>{\centering\arraybackslash}p{0.54cm}|>{\centering\arraybackslash}p{0.54cm}|>{\centering\arraybackslash}p{0.54cm}|>{\centering\arraybackslash}p{0.54cm}|>{\centering\arraybackslash}p{0.54cm}|>{\centering\arraybackslash}p{0.54cm}|>{\centering\arraybackslash}p{0.54cm}|}
\hline
N                    & 30    & 50       & 100   & 500    & 1000 & 3000 & 5000 \\ \hline
Resolution($^\circ$)        & 33.21 & 26.10 & 18.98 &  8.70 & 6.10 & 3.55 & 2.76 \\ \hline
\makecell{Time of \\Rotation(ms)} &    0.02   &    0.03      &  0.06     &   0.35    &   0.73   &    2.14    &  3.62   \\ \hline
\end{tabular}
\end{table}

==> tables/table_class.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\center
\caption{Difficulty of sensors combination to calibrate}
\label{table:class}
\begin{tabular}{cc|c|c}
\multicolumn{2}{c|}{{\color[HTML]{333333} Easy}} & {\color[HTML]{333333} Middle} & {\color[HTML]{333333} Hard} \\ \hline
64-32                 & 16-Avia                  & 64-Mid40                      & 64-radar                    \\
64-16                 & 64-Horizon               & 32-Mid40                      & Horizon-radar               \\
32-16                 & 32-Horizon               & 16-Mid40                      & Tele-radar                  \\
64-Avia               & 16-Horizon               & Horizon-Tele                  & 64-Tele                     \\
32-Avia               &                          &                               & 32-Tele                     \\
\multicolumn{2}{c|}{}                            &                               & 16-Tele                    
\end{tabular}
\end{table}

==> tables/table_init.tex <==
\begin{table}[t]
\center
\caption{Rotation Initial Results of Different Approaches in COLORFUL}
\label{table:init}

\begin{tabular}{|l|l|l|l|l|l|}
\hline
                        & Method       & Hand-Eye & FPFH & COORN & Our    \\ \hline
\multirow{3}{*}{Easy}   & 64-32        &          &      & 1.886  & 1.914  \\
                        & 32-16        &          &      & 2.262 & 2.102  \\
                        & 32-Horizon   &          &      &       & 1.612  \\ \hline
\multirow{3}{*}{Middle} & Horizon-Tele &          &      &       & 0.352  \\
                        & 32-Mid40     &          &      &       & 5.562  \\
                        & 16-Mid40     &          &      &       & 4.755 \\ \hline
\multirow{2}{*}{Hard}   & 32-Tele      &          &      &       & 4.304 \\
                        & 16-Tele      &          &      &       & 5.651 \\ \hline
                        & Mean         &          &      &       &        \\ \hline
\end{tabular}
\end{table}

==> tables/table_quan.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\center
\caption{Calibration Results of Different Approaches in COLORFUL. \\The initial value is ground truth with $2m$ and $5^\circ$ translation and rotation disturbance.}
% \label{table:refine_simu}

\begin{tabular}{|c|cc|cc|cc|cc|cc|cc|}
\hline
\multirow{2}{*}{Target} & \multicolumn{2}{c|}{MLOAM~\cite{mloam}}         & \multicolumn{2}{c|}{CROON~\cite{CROON}}         & \multicolumn{2}{c|}{Liu et al.~\cite{small_fov}}    & \multicolumn{2}{c|}{scan-scan}     & \multicolumn{2}{c|}{\je}      & \multicolumn{2}{c|}{\ho}          \\ \cline{2-13} 
                        & \multicolumn{1}{c|}{$e_{rot}$} & $e_{trans}$ & \multicolumn{1}{c|}{$e_{rot}$} & $e_{trans}$ & \multicolumn{1}{c|}{$e_{rot}$} & $e_{trans}$ & \multicolumn{1}{c|}{$e_{rot}$} & $e_{trans}$ & \multicolumn{1}{c|}{$e_{rot}$} & $e_{trans}$ & \multicolumn{1}{c|}{$e_{rot}$} & $e_{trans}$ \\ \hline
64-32                   & \multicolumn{1}{c|}{}     &        & \multicolumn{1}{c|}{}     &        & \multicolumn{1}{c|}{}     &        & \multicolumn{1}{c|}{0.0106}     &  0.0030   & \multicolumn{1}{c|}{ 0.0060}     & 0.0019  & \multicolumn{1}{c|}{}     &        \\ \hline
32-16                   & \multicolumn{1}{c|}{}     &        & \multicolumn{1}{c|}{}     &        & \multicolumn{1}{c|}{}     &        & \multicolumn{1}{c|}{0.2901}     &    0.0824    & \multicolumn{1}{c|}{0.0655}     & 0.0088& \multicolumn{1}{c|}{}     &        \\ \hline
Horizon-Tele            & \multicolumn{1}{c|}{}     &        & \multicolumn{1}{c|}{}     &        & \multicolumn{1}{c|}{}     &        & \multicolumn{1}{c|}{0.0621}     &   0.0540  & \multicolumn{1}{c|}{0.0177}     &   0.0204  & \multicolumn{1}{c|}{}     &        \\ \hline
64-Horizon                 & \multicolumn{1}{c|}{}     &        & \multicolumn{1}{c|}{}     &        & \multicolumn{1}{c|}{}     &        & \multicolumn{1}{c|}{0.0732}     &  0.0212   & \multicolumn{1}{c|}{0.0058}     &  0.0040 & \multicolumn{1}{c|}{}     &        \\ \hline
32-Mid40                & \multicolumn{1}{c|}{}     &        & \multicolumn{1}{c|}{}     &        & \multicolumn{1}{c|}{}     &        & \multicolumn{1}{c|}{0.1111}     & 0.0265  & \multicolumn{1}{c|}{0.0353}     & 0.0130 & \multicolumn{1}{c|}{}     &        \\ \hline
64-Tele               & \multicolumn{1}{c|}{}     &        & \multicolumn{1}{c|}{}     &        & \multicolumn{1}{c|}{}     &        & \multicolumn{1}{c|}{0.0801}     & 0.0779 & \multicolumn{1}{c|}{0.1021}     & 0.0664  & \multicolumn{1}{c|}{}     &        \\ 
\hline
\end{tabular}
\end{table*}

==> tables/table_refine_realword.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\center
\caption{The rotation initial result of \sd in the real-world dataset}
\label{table:refine_real_table}
\scriptsize
\begin{tabular}{|c|c|cc|cc|}
\hline
\multirow{2}{*}{Dataset} & \multirow{2}{*}{LiDAR-pair} & \multicolumn{2}{c|}{Scancontext*}               & \multicolumn{2}{c|}{\sd} \\ \cline{3-6} 
                         &                             & \multicolumn{1}{c|}{$e_{rot}$($^\circ$)} & $SR$(\%) & \multicolumn{1}{c|}{$e_{rot}$($^\circ$)} & $SR$(\%) \\ \hline
Campus1                  & \makecell{ RS-LiDAR-M1\\  LIVOX-AVIA}         & \multicolumn{1}{c|}{/ }         &   0     & \multicolumn{1}{c|}{1.144}      &  100   \\ \hline
\multirow{2}{*}{Campus2}  & \makecell{ RS-Helios(top)\\  RS-Helios(back)}          & \multicolumn{1}{c|}{7.491}          &  46.46 & \multicolumn{1}{c|}{1.521}          &  100  \\ \cline{2-6} 
                          & \makecell{ RS-Helios(top)\\ RS-Bpearl(right)} & \multicolumn{1}{c|}{/}          &    0 & \multicolumn{1}{c|}{2.243}          &  100     \\ \hline
\makecell{ USTC\\ FLICAR} & \makecell{ Ouster OS0-128\\ VLP-32C}               & \multicolumn{1}{c|}{/}          &    0    & \multicolumn{1}{c|}{3.178}          &  63.54  \\ \hline
\multirow{3}{*}{TIERS}   & \makecell{ LIVOX Horizon\\  LIVOX AVIA }                      & \multicolumn{1}{c|}{2.643}          & 66.67   & \multicolumn{1}{c|}{2.018}          &  100   \\ \cline{2-6} 
                         & \makecell{   OS-1 \\  LIVOX AVIA }                  & \multicolumn{1}{c|}{4.84}          &  21.73  & \multicolumn{1}{c|}{1.918}          &  100   \\ \cline{2-6} 
                         & \makecell{  OS-0 \\  OS-1  }                & \multicolumn{1}{c|}{4.008}          &   67.57  & \multicolumn{1}{c|}{0.5819}          &  100   \\ \hline
Pandaset                 & \makecell{  Pandar64\\  PandarGT }                        & \multicolumn{1}{c|}{5.399}          &  92.40  & \multicolumn{1}{c|}{1.438}          & 93.67 \\ \hline
A2D2                     & \makecell{  frontcenter\\  frontleft}       & \multicolumn{1}{c|}{/}          & 0  & \multicolumn{1}{c|}{8.726}          & 61.37  \\ \hline
UrbanNav                 & \makecell{  VLP16\\   Lslidar C16}                  & \multicolumn{1}{c|}{/}          &  0 & \multicolumn{1}{c|}{3.785}          & 67.78  \\ \hline
\end{tabular}
\end{table}


==> tables/table_simu.tex <==
\begin{table}[h]
\label{table_simu}
\begin{tabular}{lccccccc}
Error( m | du ) & \multicolumn{1}{l}{VLP-64} & \multicolumn{1}{l}{VLP-32} & \multicolumn{1}{l}{VLP-16} & \multicolumn{1}{l}{Front-left} & \multicolumn{1}{l}{Front-right} & \multicolumn{1}{l}{Left} & \multicolumn{1}{l}{Right} \\
VLP-64          & \textbackslash{}           & 0|0                        & 0|0                        & 0|0                            & 0|0                             & 0|0                      & 0|0                       \\
VLP-32          &                            & \textbackslash{}           & 0|0                        & 0|0                            &                                 &                          &                           \\
VLP-16          &                            &                            & \textbackslash{}           &                                &                                 &                          &                           \\
Front-left      &                            &                            &                            & \textbackslash{}               &                                 &                          &                           \\
Front-right     &                            &                            &                            &                                & \textbackslash{}                &                          &                           \\
Left            &                            &                            &                            &                                &                                 & \textbackslash{}         &                           \\
Right           &                            &                            &                            &                                &                                 &                          & \textbackslash{}         
\end{tabular}
\end{table}

==> tables/table_success.tex <==
\begin{table}[t]
\center
\caption{Success Rate}
\label{table_dataset}
\begin{tabular}{|c|c|c|}
\hline
Split  & Scan-Scan & Dsec    \\ \hline
Eazy   & 93.48\%   & 97.11\% \\ \hline
Middle & 33.13\%   & 57.50\% \\ \hline
Hard   & 6.67\%   & 20.13\% \\ \hline
\end{tabular}
\end{table}

==> tables/table_translation.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\center
\caption{The impact of translation on the \sd's precision}
\label{table:translation}
\renewcommand{\arraystretch}{1.5}
\begin{tabularx}{\linewidth}{|>{\centering\arraybackslash}Xl|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|}
\hline
\multicolumn{2}{|l|}{Translation}                          & 0 & 2 & 4 & 6 & 8 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{64-32}}   & $e_{rot}$($^\circ$) &0.001 &1.51&2.56& 3.741&2.7868\\ \cline{2-7} 
\multicolumn{1}{|l|}{}                         & $SR$(\%)            & 99.3  &100 & 83.7&34.8&29.2\\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{64-avia}} & $e_{rot}$($^\circ$) &0&0.623&1.472& 1.278&0.8660\\ \cline{2-7} 
\multicolumn{1}{|l|}{}                         & $SR$(\%)            & 100 &100&78.4&84.51& 87.632\\ \hline
\end{tabularx}
\renewcommand{\arraystretch}{1}
\end{table}
